Neural Architectural Backdoors

This paper asks the intriguing question: is it possible to exploit neural architecture search (NAS) as a new attack vector to launch previously improbable attacks? Specifically, we present EVAS, a new attack that leverages NAS to find neural architectures with inherent backdoors and exploits such vulnerability using input-aware triggers. Compared with existing attacks, EVAS demonstrates many interesting properties: (i) it does not require polluting training data or perturbing model parameters; (ii) it is agnostic to downstream fine-tuning or even re-training from scratch; (iii) it naturally evades defenses that rely on inspecting model parameters or training data. With extensive evaluation on benchmark datasets, we show that EVAS features high evasiveness, transferability, and robustness, thereby expanding the adversary's design spectrum. We further characterize the mechanisms underlying EVAS, which are possibly explainable by architecture-level ``shortcuts'' that recognize trigger patterns. This work raises concerns about the current practice of NAS and points to potential directions to develop effective countermeasures.

==> NAS backdoor/abstract.tex <==

\begin{abstract}
%Automated machine learning (AutoML) represents a new paradigm of applying ML in practice, which automates the pipeline from raw data to deployable models and enables ordinary users to readily develop and use ML techniques. Yet, despite its surging popularity, the potential security risks of \automl are largely unexplored, which is concerning given the increasing use of \automl-generated models in security-critical domains. 

This paper asks the intriguing question: {\em is it possible to exploit neural architecture search (NAS) as a new attack vector to launch previously improbable attacks?} Specifically, we present \attack, a new attack that leverages NAS to find neural architectures with inherent backdoors and exploits such vulnerability using input-aware triggers. Compared with existing attacks, \attack demonstrates many interesting properties: \mct{i} it does not require polluting training data or perturbing model parameters; \mct{ii} it is agnostic to downstream fine-tuning or even re-training from scratch; \mct{iii} it naturally evades defenses that rely on inspecting model parameters or training data. With extensive evaluation on benchmark datasets, we show that \attack features high evasiveness, transferability, and robustness, thereby expanding the adversary's design spectrum. We further characterize the mechanisms underlying \attack, which are possibly explainable by architecture-level ``shortcuts'' that recognize trigger patterns. This work raises concerns about the current practice of NAS and points to potential directions to develop effective countermeasures.
\end{abstract}


==> NAS backdoor/background.tex <==

\section{Preliminaries}
\label{sec:background}

We first introduce a set of key concepts and assumptions. 
%Table\mref{tab:notations} summarizes the important notations.

% \subsection{Neural Architecture Search}

% Deep neural networks (\dnns) represent a class of \ml models to learn high-level abstractions of complex data. We assume a predictive setting, in which a \dnn $\ssub{f}{\theta}$ (parameterized by $\theta$) encodes a function $\ssub{f}{\theta}: \ssup{\sR}{n} \rightarrow \ssup{\sS}{m}$, where $n$ and $m$ denote the input dimensionality and the number of classes. Given input $x$, $f(x)$ is a probability vector (simplex) over $m$ classes. 

% In this paper, we mainly focus on one primary task of \automl, 

% Neural architecture search (\nas) searches for performant \dnn architectures for given tasks~\citep{automl-survey}. Formally, let $\gD$ be the given dataset, $\ell(\cdot, \cdot)$ be the loss function, $\gF$ be the functional space of possible models (\mie, search space), the \nas method $\emA$ searches for a performant \dnn $\ssup{f}{*}$ via minimizing the following objective: 
% \begin{equation}
% \ssup{f}{*} = \arg\min_{f \in \gF} \E_{(x, y) \sim \gD} \, \ell(f(x), y)
% \end{equation}

% The existing \nas methods can be categorized according to their search spaces and strategies. In the following, we focus on the space of cell-based architectures~\citep{nasnet,enas,darts,snas,amoebanet}, which repeat the motif of a cell structure in a pre-specified arrangement, and the strategy of differentiable \nas\citep{darts,sgas,drnas}, which jointly optimizes the architecture and model parameters using gradient descent, due to their state-of-the-art performance and efficiency. % Nevertheless, our discussion generalizes to alternative \nas frameworks (details in \msec{sec:literature}). 
% We use {\darts}~\citep{darts} as a concrete example to illustrate differentiable \nas. 
% At a high level, \darts searches for two cell structures (\mie, normal cell and reduction cell) as the basic building blocks of the final architecture. A cell is modeled as a directed acyclic graph, in which each node $\ssup{x}{(i)}$ is a latent representation and each directed edge $(i,j)$ represents an operation $\ssup{o}{(i,j)}$ applied on $\ssup{x}{(i)}$ (\meg, skip connect). Each node is computed based on all its predecessors:
% \begin{equation}
%     \ssup{x}{(j)} = \sum_{i < j} \ssup{o}{(i,j)}(\ssup{x}{(i)})
% \end{equation}
% Each cell contains $\ssub{n}{\mathrm{in}}$ input nodes (often $\ssub{n}{\mathrm{in}}=2$), $\ssub{n}{\mathrm{out}}$ output nodes (often $\ssub{n}{\mathrm{out}} = 1$), and $\ssub{n}{\mathrm{mid}}$ intermediate nodes. Each input node takes the output from a preceding cell, the output node aggregates the latent representations from intermediate nodes, while each intermediate node is connected to $m$ preceding nodes (typically $m = \ssub{n}{\mathrm{in}}$). 
% %\ren{The illustration about intermediate nodes is confusing.}

% To enable gradient-based optimization of the architecture, \darts applies continuous relaxation on the search space. Letting $\gO$ be the set of candidate operations, the categorical choice of an operation is reduced to a softmax over $\gO$: 
% \begin{equation}
% \label{eq:softmax}
%     \ssup{\bar{o}}{(i,j)}(x) = \sum_{o \in \gO} \frac{\exp (\sboth{\alpha}{o}{(i,j)}) }{\sum_{o' \in \gO} \exp( \sboth{\alpha}{o'}{(i,j)})} o(x) 
% \end{equation}
% where $\sboth{\alpha}{o}{(i,j)}$ represents the trainable weight of operation $o$. When the search completes, a discrete architecture is obtained by replacing $\ssup{\bar{o}}{(i,j)}$ with the most likely operation $\arg\max_o \sboth{\alpha}{o}{(i,j)}$.

% The search is thus formulated as a bi-level optimization objective function: 
% \begin{equation}
% \label{eq:search}
% \min_\alpha\; \ssub{\gL}{\mathrm{val}} ( \ssup{\theta}{*}(\alpha), \alpha )    \quad \mathrm{s.t.} \quad \ssup{\theta}{*}(\alpha) = \arg\min_\theta \; \ssub{\gL}{\mathrm{trn}} (\theta, \alpha) 
% \end{equation}
% where $\ssub{\gL}{\mathrm{trn}}$ and $\ssub{\gL}{\mathrm{val}}$ are the training and validation losses, and $\alpha = \{\ssup{\alpha}{(i,j)}\}$ and  $\theta$ denote the architecture and model parameters, respectively. To handle the prohibitive cost of the nested optimization, single-step gradient descent is applied to avoid solving the inner objective exactly.
%while in {\drnas}\mcite{drnas}, the architecture parameters are modeled using a Dirichlet distribution to facilitate the optimization.

\subsection{Neural Tangent Kernel}




In \nas, it is necessary to evaluate the performance of candidate models. A na\"{i}ve way is to train the model from scratch to assess its performance, which can be extremely expensive. Recent work~\citep{nas-no-train,Wu:icea:2021,Abdelfattah:iclr:2021,Ning:nips:2021} has explored using easy-to-compute metrics as a proxy (without actual training). Most relevant to us, Chen {\em et al.} apply {\em neural tangent kernel} (NTK) to estimate the model ``trainability'' in terms of how fast the model training converges~\citep{ntk-metric}. 

Specifically, NTK describes the dynamics of DNN training by gradient descent~\citep{ntk,wide-dnn}. On the infinite width limit of DNNs, NTK becomes constant, which allows closed-form statements to be made about model training. Formally, considering given model $f$ (parameterized by $\theta$) as a map from input $x$ to a probability vector $f(x; \theta)$ over different classes, its Jacobian is defined as:
\begin{equation}
    J(x, \theta) \triangleq \frac{\partial f(x;\theta)}{\partial \theta}
\end{equation}
The NTK is then defined as the square matrix of: 
\begin{equation}
    \Theta(x, \theta) \triangleq J J^\intercal
\end{equation}
In practice, the condition number $\kappa = \frac{\lambda_{max}}{\lambda_{min}}$ of the empirical NTK matrix $\hat{\Theta}(\theta) \triangleq \E_{(x,y) \sim \gD} \Theta(x, \theta)$ is used as a metric to estimate the model trainability~\citep{ntk-metric}, with smaller conditional numbers indicating higher trainability. 
    

% by calculating its condition number. We design our attack based on this metric because it is differentiable w.r.t. model parameters.


% Neural Tangent Kernel (NTK) has been well studied to describe the dynamic evolution of DNNs during training stages).

% We have model $f$ that maps input $x$ and model parameters $\theta \in \mathbb{R}^{D}$ to a classification probability vector $f(x;\theta) \in \mathbb{R}^C$, where $C$ is number of classes.

% Jacobian
% $J(x, \theta) \triangleq \frac{\partial f(x;\theta)}{\partial \theta}$
% is a $(C\times D)$ matrix.

% Neural Tangent Kernel $\Theta(x, \theta) \triangleq J J^T$. It's a square matrix with shape $(C\times C)$.



% We evaluate the condition number $\kappa = \frac{\lambda_{max}}{\lambda_{min}}$ of empirical NTK matrix $\hat{\Theta}(\theta) \triangleq \mathbb{E}_{(x,y) \sim \mathcal{T}} [\Theta(x, \theta)]$



==> NAS backdoor/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This work studies the feasibility of exploiting \nas as an attack vector to launch previously improbable attacks. We present  a new backdoor attack that leverages \nas to efficiently find neural network architectures with inherent, exploitable vulnerability. Such architecture-level backdoors demonstrate many interesting properties including evasiveness, transferability, and robustness, thereby greatly expanding the design spectrum for the adversary. We believe our findings raise concerns about the current practice of \nas in security-sensitive domains and point to potential directions to develop effective mitigation.


% Further, we discuss potential remedies to mitigate such limitations, which sheds light on designing and operating \nas in a more robust and principled manner.


% systematic study on the security risks incurred by \automl. From both empirical and analytical perspectives, we demonstrate that \nas-generated models tend to suffer greater vulnerability to various malicious manipulations, compared with their manually designed counterparts, which implies the existence of fundamental drawbacks in the design of existing \nas methods. We identify high loss smoothness and low gradient variance, stemming from the preference of \nas for models with higher trainability, as possible causes for such phenomena. 



==> NAS backdoor/evaluation.tex <==

\section{Evaluation}
\label{sec:evaluation}

We conduct an empirical evaluation of \attack on benchmark datasets under various scenarios. The experiments are designed to answer the following key questions: \mct{i} {\em does it work?} -- we evaluate the performance and vulnerability of the arches identified by \attack; \mct{ii} {\em how does it work?} -- we explore the dynamics of \attack search as well as the characteristics of its identified arches; and \mct{ii} {\em how does it differ?} -- we compare \attack with conventional backdoors in terms of attack evasiveness, transferability, and robustness. 


\subsection{Experimental Setting}

% We first introduce the setting of the empirical evaluation. 

{\bf Datasets.} In the evaluation, we primarily use three datasets that have been widely used to benchmark NAS methods~\citep{pdarts,sgas,darts,enas,snas}: {\cifar}~\citep{cifar}, which consists of 32$\times$32 color images drawn from 10 classes; {\cifarn}, which is similar to CIFAR10 but includes 100 finer-grained classes; and {\imgnet}, which is a subset of the ImageNet dataset~\citep{imgnet} down-sampled to images of size 16$\times$16 in 120 classes. 
% {\bf Datasets --} In the evaluation, we primarily use 3 datasets that have been widely used to benchmark \nas performance in recent work\mcite{pdarts,sgas,darts,enas,snas}: {\cifar}\mcite{cifar} -- it consists of $32\times 32$ color images drawn from 10 classes (\meg, `airplane'); {\cifarn} -- it is essentially the \cifar dataset but divided into 100 fine-grained classes; {\imgnet} -- it is a subset of the ImageNet dataset\mcite{imgnet}, downsampled to images of size $16 \times 16$ in 120 classes. 

{\bf Search space.} We consider the search space defined by \nats (\mcite{Dong:tpami:2021}), which consists of 5 operators \{{\em none}, {\em skip connect}, {\em conv $1\times1$}, {\em conv $3\times3$}, and {\em avg pooling $3\times3$}\} defined among 4 nodes, implying a search space of 15,625 candidate arches.

{\bf Baselines.} We compare the arches found by \attack with ResNet18~\citep{resnet}, a  manually designed arch. For completeness, we also include two arches randomly sampled from the \nats space, which are illustrated in Figure~\ref{fig:arch}.

{\bf Metrics.} We mainly use two metrics, attack success rate (ASR) and clean data accuracy (ACC). Intuitively, ASR is the target model's accuracy in classifying trigger inputs to the adversary's target class during inference, which measures the attack effectiveness, while ACC is the target model's accuracy in correctly classifying clean inputs, which measures the attack evasiveness.


The default parameter setting and the trigger generator configuration are deferred to Appendix\,\msec{sec:appb}.

% All the models are trained using the following setting: epochs = 10, batch size = 96, optimizer = SGD, learning rate = 0.01.


\subsection{Q1: Does \attack work?}
\label{sec:analysis}

Figure~\ref{fig:arch} illustrates one sample arch identified by \attack on the \cifar dataset. We use this arch throughout this set of experiments to show that its vulnerability is at the arch level and universal across datasets. To measure the vulnerability of different arches, we first train each arch using clean data, then train a trigger generator specific to this arch, and finally measure its ASR and ACC. 



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/arch.pdf}
    \caption{Sample arch identified by \attack in comparison of two randomly generated arches. \label{fig:arch}}
\end{figure}

Table~\ref{tab:direct} reports the results. We have the following observations. First, the ASR of \attack is significantly higher than ResNet18 and the other two random arches. For instance, on \cifar, \attack is 21.8\%, 28.3\%, and 34.5\% more effective than ResNet18 and random arches, respectively. 
%55.83\% ASR while the ASR of ResNet is 42.28\%, which is 13.55\% difference. The 2 random architectures are with 37.45\% and 32.15\%. The high attack successful rate proves the effectiveness of \attack. 
Second, \attack has the highest ASR across all the datasets. Recall that we use the same arch throughout different datasets. This indicates that the attack vulnerability probably resides at the arch level and is agnostic to concrete datasets. Third, all the arches show higher ASR on simpler datasets such as \cifar. This may be explained by  that more complex datasets (\meg, more classes, higher resolution) imply more intricate manifold structures, which may interfere with arch-level backdoors. 






% \subsubsection{Setting 1: Direct use of an original model}
% \label{sec:direct}
% In this first setting, the user directly uses a clean model which the attack has access to without fine-tuning or re-training. We compare the performance of \attack with ResNet and 2 random architectures from \nats on \cifar, \cifarn and \imgnet datasets and report the results in Table~\ref{tab:direct}. We have the following observations. First, attack successful rate on \attack is higher than ResNet and the other 2 random architectures. For instance, on \imgnet, \attack has 55.83\% ASR while the ASR of ResNet is 42.28\%, which is 13.55\% difference. The 2 random architectures are with 37.45\% and 32.15\%. The high attack successful rate proves the effectiveness of \attack. Second, across all datasets, \cifar has the highest attack successful rate. Compared with the 81.51\% ASR on \cifar, the ASR on \imgnet is only 55.83\%. It could be explained by the fewer classes and higher image resolution in \cifar classification task.

\begin{table}[!ht]{\footnotesize
    \renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3pt}
    \caption{Model performance on clean inputs (ACC) and attack performance on trigger-embedded inputs (ASR) of \attack, ResNet18, and two random arches. \label{tab:direct}}
\begin{center}
    \begin{tabular}{c|c c|c c|c c|c c}
    \multirow{3}{*}{dataset} & \multicolumn{8}{c}{architecture} \\
    \cline{2-9}
    & \multicolumn{2}{c|}{\attack} & \multicolumn{2}{c|}{ResNet18} & \multicolumn{2}{c|}{Random I} & \multicolumn{2}{c}{Random II} \\
    \cline{2-9}
    & ACC & ASR & ACC & ASR & ACC & ASR & ACC & ASR \\
    \hline
    \cifar & 94.26\% & \cellcolor{Red}81.51\% & 96.10\% & 59.73\% & 91.91\% & 53.21\% & 92.05\% & 47.04\% \\
    \cifarn & 71.54\% & \cellcolor{Red}60.97\% & 78.10\% & 53.53\% & 67.09\% & 42.41\% & 67.15\% & 47.17\% \\
    \imgnet & 45.92\% & \cellcolor{Red}55.83\% & 47.62\% & 42.28\% & 39.33\% & 37.45\% & 39.48\% & 32.15\% \\
    \end{tabular}
\end{center}}
\end{table}

% Further, to evaluate whether \attack is sensitive to the target class set by the adversary, we measure its ASR under different target classes, with results shown in Table~\ref{tab:class}.

% \begin{table*}[!ht]{\footnotesize
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%   \setlength{\tabcolsep}{3pt}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%     Class & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
%     \hline
%     ASR & 81.75\% & 65.06\% & 61.00\% & 72.30\% & 70.70\% & 74.43\% & 67.76\% & 51.35\% & 74.21\% & 56.85\% \\
%     \end{tabular}
%     \caption{Attack Successful Rate (ASR) of \attack w.r.t. different target class on \cifar dataset. \label{tab:class}}}
% \end{table*}


% We also investigate the performance of \attack against different target classes. In previous experiments, the target class is fixed to be ``airplane''. Here we show the results w.r.t all classes on \cifar dataset in Table~\ref{tab:class}. Results show that ``airplane'' as the target class shows higher attack successful rate. A possible reason is that airplane images often has white or blue sky background composed of similar and dull colors, providing enough blank space to inject backdoor information.

To understand the attack effectiveness of \attack on individual inputs, we illustrate sample clean inputs and their trigger-embedded variants in Figure~\ref{fig:heatmap}. Further, using GradCam~\citep{selvaraju:gradcam}, we show the model's interpretation of clean and trigger inputs with respect to their original and target classes. Observe that the trigger pattern is specific to each input. Further, even though the two trigger inputs are classified to the same target class, the difference in their heatmaps shows that the model pays attention to distinct features, highlighting the effects of input-aware triggers.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/heatmap.pdf}
    \caption{Sample clean and trigger-embedded inputs as well as their GradCam interpretation by the target model. \label{fig:heatmap}}
\end{figure}


\subsection{Q2: How does \attack work?} 

Next, we explore the dynamics of how \attack searches for exploitable arches. For simplicity, given the arch identified by \attack in Figure~\ref{fig:arch}, we consider the set of candidate arches with the operators on the 0-3 ({\em skip connect}) and 0-1 ({\em conv} 3$\times$3) connections replaced by others. We measure the ACC and ASR of all these candidate arches and illustrate the landscape of their scores in Figure~\ref{fig:trajectory}. Observe that the exploitable arch features the lowest score among the surrounding arches, suggesting the existence of feasible mutation paths from random arches to reach exploitable arches following the direction of score descent. 


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/trajectory.pdf}
    \caption{Landscape of candidate arches surrounding exploitable arches with their ASR, ACC, and scores. \label{fig:trajectory}}
\end{figure}

Further, we ask the question: {\em what makes the arches found by \attack exploitable?} Observe that the arch in Figure~\ref{fig:arch} uses the {\em conv} 1$\times$1 and 3$\times$3 operators on a number of connections. We thus generate arches by enumerating all the possible combinations of {\em conv} 1$\times$1 and 3$\times$3 on these connections and measure their performance, with results summarized in Appendix\,\msec{sec:trajectory}. Observe that while all these arches show high ASR, their vulnerability varies greatly from about 50\% to 90\%. We hypothesize that specific combinations of {\em conv} 1$\times$1 and {\em conv} 3$\times$3 create arch-level ``shortcuts'' for recognizing trigger patterns. We consider exploring the causal relationships between concrete arch characteristics and attack vulnerability as our ongoing work.


\subsection{Q3: How does \attack differ?}

To further understand the difference between \attack and conventional backdoors, we compare the arches found by \attack and other arches under various training and defense scenarios.

{\bf Fine-tuning with clean data.} We first consider the scenario in which, with the trigger generator fixed, the target model is fine-tuned using clean data (with concrete setting deferred to Appendix\,\msec{sec:appb}). Table~\ref{tab:fine-tune} shows the results evaluated on \cifar and \cifarn. Observe that
fine-tuning has a marginal impact on the ASR of all the arches. Take Random I as an example, compared with  Table~\ref{tab:direct}, its ASR on \cifar drops only by 7.40\% after fine-tuning. This suggests that the effectiveness of fine-tuning to defend against input-aware backdoor attacks may be limited. 
% In conclusion, the performance fine-tuning as a mitigation against natural dynamic backdoors is limited. 
% Detailed fine-tuning parameter settings are listed in Appendix\,\msec{sec:appb}.

\begin{table*}[!ht]{\footnotesize
    \caption{Model performance on clean inputs (ACC) and attack performance on trigger-embedded inputs (ASR) of \attack, ResNet18, and two random arches after fine-tuning. \label{tab:fine-tune}}
    \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{3pt}
\begin{center}
   \begin{tabular}{c|c c|c c|c c|c c}
    \multirow{3}{*}{dataset} & \multicolumn{8}{c}{architecture} \\
    \cline{2-9}
    & \multicolumn{2}{c|}{\attack} & \multicolumn{2}{c|}{ResNet18} & \multicolumn{2}{c|}{Random I} & \multicolumn{2}{c}{Random II} \\
    \cline{2-9}
    & ACC & ASR & ACC & ASR & ACC & ASR & ACC & ASR \\
    \hline
    \cifar & 90.33\% & \cellcolor{Red}74.40\% & 92.22\% & 53.87\% & 85.62\% & 45.81\% & 87.02\% & 45.16\% \\
    \cifarn & 72.52\% & \cellcolor{Red}53.50\% & 79.02\% & 50.42\% & 58.89\% & 38.91\% & 60.18\% & 25.41\% \\
    % \imgnet & 37.05\% & 0.00\% & 41.667\% & 0.00\% & 30.20\% & 36.95\% & 29.06\% & 3.11\% \\
    \end{tabular}
\end{center}}
\end{table*}

{\bf Re-training from scratch.} Another common scenario is that the victim user re-initializes the target model and re-trains it from scratch using clean data. We simulate this scenario as follows. After the trigger generator and target model are trained, we fix the generator, randomly initialize (using different seeds) the model, and train it on the given dataset. 
%Thanks to \nats, which provides pre-trained weights for each model architecture based on 2 or 3 random seeds, we can simply evaluate attack generators from \msec{sec:analysis} on models trained with another random seed. 
Table~\ref{tab:retraining} compares different arches under this scenario. It is observed that 
\attack significantly outperforms ResNet18 and random arches in terms of ASR (with comparable ACC). For instance, it is 33.4\%, 24.9\%, and 19.6\% more effective than the other arches respectively. This may be explained by two reasons. First, the arch-level backdoors in \attack are inherently more agnostic to model re-training than the model-level backdoors in other arches. Second, in searching for exploitable arches, \attack explicitly enforces that such vulnerability should be insensitive to model initialization (\mcf \meq{eq:search}). Further, observe that, as expected, re-training has a larger impact than fine-tuning on the ASR of different arches; however, it is still insufficient to mitigate input-aware backdoor attacks.


% \cifarn, \attack shows 3.08\% higher ASR than ResNet. On the other hand, compared with 60.97\% in Table~\ref{tab:direct} and 53.50\% in Table~\ref{tab:fine-tune}, the number after re-training is only 49.47\%. This means re-training cannot totally avoid the backdoors, but somehow achieve the mitigation. 
% It is easy to understand that models trained with different random seeds have similar behaviors on clean data distribution but show very different predictions on abnormal data scopes.

\begin{table*}[!ht]{\footnotesize
    \caption{Model performance on clean inputs (ACC) and attack performance on trigger-embedded inputs (ASR) of \attack, ResNet18 and two random arches after re-training from scratch. \label{tab:retraining}}
    \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{3pt}
\begin{center}
    \begin{tabular}{c|c c|c c|c c|c c}
    \multirow{3}{*}{dataset} & \multicolumn{8}{c}{architecture} \\
    \cline{2-9}
    & \multicolumn{2}{c|}{\attack} & \multicolumn{2}{c|}{ResNet18} & \multicolumn{2}{c|}{Random I} & \multicolumn{2}{c}{Random II} \\
    \cline{2-9}
    & ACC & ASR & ACC & ASR & ACC & ASR & ACC & ASR \\
    \hline
    \cifar  & 94.18\%  & \cellcolor{Red}64.57\%  & 95.62\%  & 31.15\%  & 91.91\%  & 39.72\%  & 92.09\%  & 45.02\% \\
    \cifarn & 71.54\%  & \cellcolor{Red}49.47\%  & 78.53\%  & 44.39\%  & 67.09\%  & 35.80\%  & 67.01\%  & 39.24\% \\
    % \imgnet & 45.83\%  & 0.917\%  & 46.87\%  & 0.43\%  & 39.13\%  & 2.95\%  & 39.40\%  & 0.03\% \\
    \end{tabular}
\end{center}}
\end{table*}

% \subsubsection{Setting 4: Fine-Tuning using poisoning training data}
{\bf Fine-tuning with poisoning data.} Further, we explore the setting in which the adversary is able to poison a tiny portion of the fine-tuning data, which assumes a stronger threat model. To simulate this scenario, we apply the trigger generator to generate trigger-embedded inputs and mix them with the clean fine-tuning data. 
%Figure~\ref{{\bf Fine-tuning with poisoning datFinally, we extend the fine-tuning scenario in \msec{sec:fine-tune} that the attacker could inject a minority of poisoning data. At the proportion scale of $10^{-5}$, 
Figure~\ref{fig:poison_ratio} illustrates the ASR and ACC of the target model as functions of the fraction of poisoning data in the fine-tuning dataset. Observe that, even with an extremely small poisoning ratio (\meg, 0.01\%), it can significantly boost the ASR (\meg, 100\%) while keeping the ACC unaffected. This indicates that arch-level backdoors can be greatly enhanced by combining with other attack vectors (\meg, data poisoning). 


% reveals that the attack successful rate could get significantly boosted while clean accuracy is not sacrificed. When the poison ratio is $0$, it degenerates to the clean data case in \msec{sec:fine-tune}. We observe that there is a significant leap at $2\times 10^-5$. This is reasonable because \cifar has $50000$ training images, and a proportion of $2\times 10^-5$ guarantees that there must be 1 poisoned image for every training epoch, while it would be sampled as 0 or 1 with probability otherwise.

% \begin{table*}[!ht]{\footnotesize
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%   \setlength{\tabcolsep}{3pt}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
%     Poison Ratio & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
%     \hline
%     ASR & 75.36\% & 80.56\% & 90.29\% & 90.74\% & 91.03\% & 92.51\% & 94.65\% & 97.14\% & 99.21\% & 100.00\% & 100.00\% \\
%     ACC & 94.10\% & 94.34\% & 94.37\% & 94.33\% & 94.35\% & 94.28\% & 94.31\% & 94.34\% & 94.34\% & 94.30\% & 94.23\% \\
%     \end{tabular}
%     \caption{poisoning ratio results ($*10^{-6}$)}}
% \end{table*}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/poison_ratio.pdf}
    \caption{Model performance on clean inputs (ACC) and attack performance on trigger-embedded inputs (ASR) of \attack as a function of poisoning ratio. \label{fig:poison_ratio}}
\end{figure}

{\bf Backdoor defenses.} Finally, we evaluate \attack against three categories of defenses, model inspection, input filtering, and model sanitization. 

Model inspection determines whether a given model $f$ is infected with backdoors. We use \nc~\citep{neural-cleanse} as a representative defense. Intuitively, it searches for potential triggers in each class. If a class is trigger-embedded, the minimum perturbation required to change the predictions of inputs from other classes to this class is abnormally small. It detects anomalies using median absolute deviation (MAD) and all classes with MAD scores larger than 2 are regarded as infected. As shown in Table~\ref{tab:nc-strip}, the MAD scores of \attack's target classes on three datasets are all below the threshold. This can be explained by that \nc is built upon the universal trigger assumption, which does not hold for \attack.

\begin{table*}[!ht]{\footnotesize
    \caption{Detection results of \nc and \strip for \attack. \nc shows the MAD score and \strip shows the AUROC score of binary classification. \label{tab:nc-strip}}
    \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{4pt}
\begin{center}
    \begin{tabular}{c|c|c}
 dataset    & \nc & \strip \\
\hline    
    \cifar & 0.895 & 0.49 \\
    \cifarn & 0.618 & 0.51 \\
    \imgnet & 0.674 & 0.49 \\
    \end{tabular}
\end{center}}
\end{table*}

Input filtering detects at inference time whether an incoming input is embedded with a trigger. We use \strip~\citep{Gao:2019:arxiv} as a representative defense in this category. It mixes a given input with a clean input and measures the self-entropy of its prediction. If the input is trigger-embedded, the mixture remains dominated by the trigger and tends to be misclassified, resulting in low self-entropy. However, as shown in Table~\ref{tab:nc-strip}, the AUROC scores of \strip in classifying trigger-embedded inputs by \attack are all close to random guess (\mie, 0.5). This can also be explained by that \attack uses input-aware triggers, where each trigger only works for one specific input and has a limited impact on others.


% listed in are all nearly $0.50$, which means \strip performance is close to random guess. It could be explained by the \ren{cross-trigger term} optimized in input-aware triggers~\citep{input-aware-backdoor}, which limits the generated trigger only work for the corresponding input.

% We also verify our algorithm using backdoor defenses. In this paper, we evaluate \nc~\citep{neural-cleanse}), \fp(\mcite{Liu:2018:arxiv2}) and \strip(\mcite{Gao:2019:arxiv}), which stand for 3 main categories of backdoor defenses. \nc optimizes trigger patterns to convert all inputs to each class and check if any pattern is much smaller than others. It detects anomaly index by median absolute deviation (MAD) and all classes with MAD score larger than 2 is regarded as poisoned. As can be seen from Table~\ref{tab:nc-strip}, \attack passes the test easily. The MAD score on \cifar, \cifarn and \imgnet are all far from the threshold. This is because of 2 reasons: (i)\nc only works for detecting small universal backdoors, while the threat model is dynamic for each input image; (ii) our model is trained on clean dataset and it does not contain any small universal backdoor.



\begin{table*}[!ht]{\footnotesize
    \caption{Model performance on clean inputs (ACC) and attack performance on trigger-embedded inputs (ASR) of \attack and ResNet18 after \fp. \label{tab:fp}}
    \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{4pt}
\begin{center}
    \begin{tabular}{c|c c|c c}
    \multirow{3}{*}{dataset} & \multicolumn{4}{c}{architecture} \\
    \cline{2-5}
    & \multicolumn{2}{c|}{\attack} & \multicolumn{2}{c}{ResNet18} \\
    \cline{2-5}
    & ACC & ASR & ACC & ASR \\
    \hline
    \cifar & 90.53\% & \cellcolor{Red}72.56\% & 94.11\% & 50.95\% \\
    \cifarn & 64.92\% & \cellcolor{Red}54.55\% & 73.35\% & 38.54\% \\
    \imgnet & 40.28\% & \cellcolor{Red}32.57\% & 42.53\% & 27.59\% \\
    \end{tabular}
\end{center}}
\end{table*}

Model sanitization, before using a given model, sanitizes it to mitigate the potential backdoors, yet without explicitly detecting whether the model is tampered. We use \fp~\citep{Liu:2018:arxiv2} as a representative. It uses the property that the backdoor attack typically exploits spare model capacity. It thus prunes rarely used neurons and then applies fine-tuning to defend against pruning-aware attacks. We apply \fp on the \attack and ResNet18 models from Table~\ref{tab:direct}, with results shown in Table~\ref{tab:fp}. Observe that \fp has a limited impact on the ASR of \attack (even less than ResNet18). This may be explained as follows. The activation patterns of input-aware triggers are different from that of universal triggers, as each trigger may activate a different set of neurons. Moreover, the arch-level backdoors in \attack may not concentrate on individual neurons but span over the whole model structures. 


% Take \cifarn as an example, after \fp, the clean accuracy becomes 64.92\% and attack successful rate is 54.55\%. It is clear that clean accuracy drops but attack still works at some extent. According to \ren{heatmap results}, the activation pattern of input-aware dynamic backdoor is quite different from universal backdoors. The input neuron activation does not concentrate on the trigger pixels but scatter at the whole image because of the dynamic property.



% Another defense \fp serves as a mitigation. It removes the neurons rarely activated on clean images.
% We apply \fp on \attack and ResNet models from Table~\ref{tab:direct} and list the results in Table~\ref{tab:fp}. Take \cifarn as an example, after \fp, the clean accuracy becomes 64.92\% and attack successful rate is 54.55\%. It is clear that clean accuracy drops but attack still works at some extent. According to \ren{heatmap results}, the activation pattern of input-aware dynamic backdoor is quite different from universal backdoors. The input neuron activation does not concentrate on the trigger pixels but scatter at the whole image because of the dynamic property.

% In contrast, \strip filters poisoned inputs at test time. It mixes the test input with a clean input and assumes the backdoor pattern in the mixed input still dominates the classification results. The AUC-ROC scores of binary predictions listed in Table~\ref{tab:nc-strip} are all nearly $0.50$, which means \strip performance is close to random guess. It could be explained by the \ren{cross-trigger term} optimized in input-aware triggers~\citep{input-aware-backdoor}, which limits the generated trigger only work for the corresponding input.




==> NAS backdoor/introduction.tex <==

\section{Introduction}
\label{sec:intro}

As a new paradigm of applying ML techniques in practice, automated machine learning (\automl) automates the pipeline from raw data to deployable models, which covers model design, optimizer selection, and parameter tuning. The use of \automl greatly simplifies the \ml development cycles and propels the trend of \ml democratization. In particular, neural architecture search (\nas), one primary \automl task, aims to find performant deep neural network (\dnn) arches\footnote{In the following, we use ``arch'' for short of ``architecture''.} tailored to given datasets. In many cases, \nas is shown to find models remarkably outperforming manually designed ones~\citep{enas,darts,sgas}.


In contrast to the intensive research on improving the capability of \nas, its security implications are largely unexplored. As \ml models are becoming the new targets of malicious attacks~\citep{Biggio:2018:pr}, the lack of understanding about the risks of \nas is highly concerning, given its surging popularity in security-sensitive domains~\citep{pang:2022:sec}. Towards bridging this striking gap, we pose the intriguing yet critical question: 

\begin{center}
    {\em Is it possible for the adversary to exploit \nas to launch previously improbable attacks?}
\end{center}

This work provides an affirmative answer to this question. We present {\em exploitable and vulnerable arch search} (\attack), a new backdoor attack that leverages \nas to find neural arches with inherent, exploitable vulnerability. Conventional backdoor attacks typically embed the malicious functions (``backdoors'') into the space of model parameters. They often assume strong threat models, such as polluting training data~\citep{badnet,trojannn,evil-twin} or perturbing model parameters~\citep{model-reuse,deploy-backdoor}, and are thus subject to defenses based on model inspection~\citep{neural-cleanse,abs} and data filtering~\citep{Gao:2019:arxiv}. In \attack, however, as the backdoors are carried in the space of model arches, even if the victim trains the models using clean data and operates them in a black-box manner, the backdoors are still retained. Moreover, due to its independence of model parameters or training data, \attack is naturally robust against defenses such as model inspection and input filtering. 

To realize \attack, we define a novel metric based on neural tangent kernel~\citep{ntk-metric}, which effectively indicates the exploitable vulnerability of a given arch; further, we integrate this metric into the \nas-without-training framework~\citep{nas-no-train,ntk-metric}. The resulting search method is able to efficiently identify candidate arches without requiring model training or backdoor testing. To verify \attack's empirical effectiveness, we evaluate \attack on benchmark datasets and show: \mct{i} \attack successfully finds arches with exploitable vulnerability, \mct{ii} the injected backdoors may be explained by arch-level ``shortcuts'' that recognize trigger patterns, and \mct{iii} \attack demonstrates high evasiveness, transferability, and robustness against defenses. 
Our findings show the feasibility of exploiting \nas as a new attack vector to implement previously improbable attacks, raise concerns about the current practice of \nas in security-sensitive domains, and point to potential directions to develop effective
mitigation.


==> NAS backdoor/literature.tex <==


\section{Related Work}
\label{sec:literature}

Next, we survey the literature relevant to this work.

{\bf Neural arch search.} The existing \nas methods can be categorized along search space, search strategy, and performance measure. Search space -- early methods focus on the chain-of-layer structure~\citep{rl-automl}, while recent work proposes to search for motifs of cell structures~\citep{nasnet,enas,darts}. Search strategy -- early methods rely on either random search~\citep{random-perm} or Bayesian optimization~\citep{bayesian-nas}, which are limited in model complexity; recent work mainly uses the approaches of reinforcement learning~\citep{rl-automl} or neural evolution~\citep{darts}. Performance measure -- one-shot \nas has emerged as a popular performance measure. It considers all candidate arches as different sub-graphs of a super-net (\mie, the one-shot model) and shares weights between candidate arches~\citep{darts}. Despite the intensive research on \nas, its security implications are largely unexplored. Recent work shows that \nas-generated models tend to be more vulnerable to various malicious attacks than manually designed ones~\citep{pang:2022:sec, adversarial-robustness-arch}. This work explores another dimension: whether it can be exploited as an attack vector to launch new attacks, which complements the existing studies on the security of \nas.

{\bf Backdoor attacks and defenses.} Backdoor attacks inject malicious backdoors into the victim's model during training and activate such backdoors at inference, which can be categorized along attack targets -- input-specific~\citep{Shafahi:2018:nips}, class-specific~\citep{tact}, or any-input~\citep{badnet}, attack vectors -- polluting training data~\citep{trojannn} or releasing infected models~\citep{model-reuse}, and optimization metrics -- attack effectiveness~\citep{evil-twin}, transferability~\citep{latent-backdoor}, or attack evasiveness\citep{chen:2017:arxiv}. To mitigate such threats, many defenses have also been proposed, which can be categorized according to their strategies~\citep{trojanzoo}: input filtering purges poisoning samples from training data~\citep{Tran:2018:nips}; model inspection determines whether a given model is backdoored\citep{abs,neural-cleanse}, and input inspection detects trigger inputs at inference time~\citep{Gao:2019:arxiv}. Most attacks and defenses above focus on backdoors implemented in the space of model parameters. Concurrent to this work, \cite{arch-backdoor} explore using neural arches to implement backdoors by manually designing ``trigger detectors'' in the arches and activating such detectors using poisoning data during training. This work investigates using \nas to directly search for arches with exploitable vulnerability, which represents a new direction of backdoor attacks.

% Recently, input-aware triggers have been explored by researchers\citep{dynamic-backdoor,input-aware-backdoor}. Different from conventional backdoor attacks, input-aware triggers produce a unique trigger pattern for each input by training a backdoor generator. Up to now, there is no defense against dynamic backdoors published yet. A parallel work DECK\citep{deck} proposes a possible defense solution, which might be helpful for future dynamic backdoor research.



% \ren{Backdoor attacks have been a severe security problem since the first backdoor attack BadNet~\citep{badnet} is published. Most attack work~\citep{chen:2017:arxiv, evil-twin, Yao:2019:ccs, trojannn} is focusing on the threat model where a universal trigger pattern is applied to all inputs. According to \citep{trojanzoo}, the existing defense methods against backdoor attacks can be categorized as: \mct{i} input reformation: reforms inputs to mitigate the influence of the potential trigger~\citep{wang:cvpr:2021, Meng:2017:ccs}; \mct{ii} input filtering: detects whether an incoming input is embedded with a trigger~\citep{Gao:2019:arxiv, Chen:2018:arxiv, Tran:2018:nips}; \mct{iii} model sanitization: sanitizes the model to mitigate the potential backdoor~\citep{Liu:2018:arxiv2, pgd}; \mct{iv} model inspection: determines whether a model is a trojan model~\citep{neural-cleanse, Chen:2019:IJCAI, abs}.}

% \ren{Recently, input-aware triggers have been explored by researchers\citep{dynamic-backdoor,input-aware-backdoor}. Different from conventional backdoor attacks, input-aware triggers produce a unique trigger pattern for each input by training a backdoor generator. Up to now, there is no defense against dynamic backdoors published yet. A parallel work DECK\citep{deck} proposes a possible defense solution, which might be helpful for future dynamic backdoor research.}



% \vspace{2pt}
% {\bf ML Security --} With their wide use in security-sensitive domains, ML models are becoming the new targets for malicious manipulations\mcite{Biggio:2018:pr}. A variety of attack vectors have been exploited: adversarial evasion crafts adversarial inputs to force the target model to misbehave\mcite{goodfellow:fsgm,carlini-attack}; model poisoning modifies the target model's behavior (\meg, performance drop) via polluting its training data\mcite{model-reuse}; backdoor injection creates a trojan model such that any input embedded with a specific trigger is likely to be misclassified by the model\mcite{badnet,trojannn}; functionality stealing constructs a replicate model functionally similar to a victim model\mcite{knockoff-net,hardware-model-stealing}; membership inference breaches data privacy via inferring whether a given input is included in the model's training data based on the model's prediction\mcite{membership-attack}.

% In response, another line of work strives to improve the resilience of ML models against such attacks. For instance, against adversarial evasion, existing defenses explore new training strategies (\meg, adversarial training)\mcite{pgd,Tramer:2018:iclr} and detection mechanisms\mcite{Meng:2017:ccs,Gehr:2018:sp}. Yet, such defenses often fail when facing even stronger attacks\mcite{Athalye:2018:icml,deepsec}, resulting in a constant arms race between the attackers and defenders.


% \ting{rewrite this paragraph}
% Despite the intensive research on \nas and \ml security in parallel, the robustness of \nas-generated models to malicious manipulations is fairly under-explored\mcite{robust-nas}. Concurrent to this work, it is shown in\mcite{pang:2022:sec, adversarial-robustness-arch} that \nas models tend to be more vulnerable to adversarial evasion, while our work differs in considering a variety of attacks beyond adversarial evasion, providing possible explanations for such vulnerability, and investigating potential mitigation.

%This work bridges this gap by conducting the first study on the security risks incurred by \nas, which raises concerns for the current practice of \automl in general.


==> NAS backdoor/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> NAS backdoor/method.tex <==

\section{\attack}

Next, we present \attack, a new backdoor attack leveraging \nas to find neural arches with exploitable vulnerability. We begin by introducing the threat model.


\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/archbkd.pdf}
    \caption{Attack framework of \attack. \mct{1} The adversary applies \nas to search for arches with exploitable vulnerability; \mct{2} such vulnerability is retained even if the models are trained using clean data; \mct{3} the adversary exploits such vulnerability by generating trigger-embedded inputs.
    \label{fig:archbkd}}
\end{figure}

\subsection{Threat Model}

A backdoor attack injects a hidden malicious function (``backdoor'') into a target model~\citep{trojanzoo}. The backdoor is activated once a pre-defined condition (``trigger'') is present, while the model behaves normally otherwise. In a predictive task, the backdoor is often defined as classifying a given input to a class desired by the adversary, while the trigger can be defined as a specific perturbation applied to the input. Formally, given input $x$ and trigger $r = (m, p)$ in which $m$ is a mask and $p$ is a pattern, the trigger-embedded input is defined as:
\begin{equation}
    \tilde{x} =  x \odot (1-m) + p \odot m
\end{equation}
Let $f$ be the backdoor-infected model. The backdoor attack implies that for given input-label pair $(x, y)$, $f(x) = y$ and $f(\tilde{x}) = t$ with high probability, where $t$ is the adversary's target class. 


The conventional backdoor attacks typically follow two types of threat models: \mct{i} the adversary directly trains a backdoor-embedded model, which is then released to and used by the victim user~\citep{trojannn,evil-twin,model-reuse}; or \mct{ii} the adversary indirectly pollutes the training data or manipulate the training process~\citep{badnet,deploy-backdoor} to inject the backdoor into the target model. As illustrated in Figure~\ref{fig:archbkd}, in \attack, we assume a more practical threat model in which the adversary only releases the exploitable arch to the user, who may choose to train the model using arbitrary data (\meg, clean data) or apply various defenses (\meg, model inspection or data filtering) before or during using the model. We believe this represents a more realistic setting: due to the prohibitive computational cost of \nas, users may opt to use performant model arches provided by third parties, which opens the door for the adversary to launch the \attack attack.

However, realizing \attack represents non-trivial challenges including \mct{i} how to define the trigger patterns? \mct{ii} how to define the exploitable, vulnerable arches? and \mct{iii} how to search for such arches efficiently? Below we elaborate on each of these key questions. 

\subsection{Input-Aware Triggers}

Most conventional backdoor attacks assume universal triggers: the same trigger is applied to all the inputs. However, universal triggers can be easily detected and mitigated by current defenses~\citep{neural-cleanse,abs}. Moreover, it is shown that implementing universal triggers at the arch level requires manually designing ``trigger detectors'' in the arches and activating such detectors using poisoning data during training~\citep{arch-backdoor}, which does not fit our threat model.

Instead, as illustrated in Figure~\ref{fig:archbkd}, we adopt input-aware triggers~\citep{input-aware-backdoor}, in which a trigger generator $g$ (parameterized by $\vartheta$) generates trigger $r_x$ specific to each input $x$. Compared with universal triggers, it is more challenging to detect or mitigate input-aware triggers. Interestingly, because of the modeling capacity of the trigger generator, it is more feasible to implement input-aware triggers at the arch level (details in \msec{sec:evaluation}). For simplicity, below we use $\tilde{x} = g(x;\vartheta)$ to denote both generating trigger $r_x$ for $x$ and applying $r_x$ to $x$ to generate the trigger-embedded input $\tilde{x}$.

\subsection{Exploitable arches} 

In \attack, we aim to find arches with backdoors exploitable by the trigger generator, which we define as the following optimization problem.

Specifically, let $\alpha$ and $\theta$ respectively denote $f$'s arch and model parameters. We define $f$'s training as minimizing the following loss:
\begin{equation}
\gL_\mathsf{trn} (\theta, \alpha)  \triangleq \E_{(x, y) 
\sim \gD}  \ell (f_\alpha(x; \theta), y) 
\end{equation}
where $f_\alpha$ denotes the model with arch fixed as $\alpha$ and $\gD$ is the underlying data distribution. As $\theta$ is dependent on $\alpha$, we define: 
\begin{equation}
\theta_\alpha \triangleq \arg\min_\theta \gL_\mathsf{trn} (\theta, \alpha)
\end{equation}
Further, we define the backdoor attack objective as: 
\begin{equation}
\label{eq:search}
\gL_\mathsf{atk} (\alpha, \vartheta) \triangleq \E_{(x, y) \sim \gD} \, [\ell (f_\alpha(x; \theta_\alpha) , y)
+ \lambda \ell (f_\alpha( g(x;\vartheta); \theta_\alpha), t)]
\end{equation}
where the first term specifies that $f$ works normally on clean data, the second term specifies that $f$ classifies trigger-embedded inputs to target class $t$, and the parameter $\lambda$ balances the two factors. Note that we assume the testing data follows the same distribution $\gD$ as the training data.

Overall, we consider an arch $\alpha^*$ having exploitable vulnerability if it is possible to find a trigger generator $\vartheta^*$, such that $\gL_\mathsf{atk} (\alpha^*, \vartheta^*)$ is below a certain threshold.

% Overall, we formulate the search for vulnerable archs as a bi-level optimization objective: 
% \begin{equation}
% \label{eq:search}
% \min_{\alpha, \vartheta} \gL_\mathsf{atk} ( \theta_\alpha, \alpha, \vartheta)    \quad \mathrm{s.t.} \quad \theta_\alpha = \arg\min_\theta \gL_\mathsf{trn} (\theta, \alpha) 
% \end{equation}
% Note that $\alpha$ and $\vartheta$ are coupled in $\gL_\mathsf{atk}$.

\subsection{Search without Training}  

Searching for exploitable archs by directly optimizing \meq{eq:search} is challenging: the nested optimization requires recomputing $\theta$ (\mie, re-training model $f$) in $\gL_\mathsf{trn}$ whenever $\alpha$ is updated; further, as $\alpha$ and $\vartheta$ are coupled in $\gL_\mathsf{atk}$, it requires re-training generator $g$ once $\alpha$ is changed. 

Motivated by recent work~\citep{nas-no-train,Wu:icea:2021,Abdelfattah:iclr:2021,Ning:nips:2021} on \nas using easy-to-compute metrics as proxies (without training), we present a novel method of searching for exploitable arches based on {\em neural tangent kernel} (NTK)~\citep{ntk} without training the target model or trigger generator. 
% has explored using easy-to-compute metrics as a proxy (without actual training). Most relevant to us, Chen {\em et al.} apply {\em neural tangent kernel} (NTK) to estimate the model ``trainability'' in terms of how fast the model training converges~\citep{ntk-metric}. 
Intuitively, NTK describes model training dynamics by gradient descent~\citep{ntk}. On the infinite width limit of DNNs, NTK becomes constant, which allows closed-form statements to be made about model training~\citep{wide-dnn}. Formally, considering model $f$ (parameterized by $\theta$) mapping input $x$ to a probability vector $f(x; \theta)$ (over different classes), the NTK is defined as the product of the Jacobian matrix:
\begin{equation}
    \Theta(x, \theta) \triangleq \left[\frac{\partial f(x;\theta)}{\partial \theta}\right] \left[\frac{\partial f(x;\theta)}{\partial \theta}\right]^\intercal %\quad J(x, \theta) \triangleq \frac{\partial f(x;\theta)}{\partial \theta}
\end{equation}
% The NTK is then defined as the square matrix of: 
% \begin{equation}
% \end{equation}
Let $\lambda_\mathrm{min}$ ($\lambda_\mathrm{max}$) be the smallest (largest) eigenvalue of the empirical NTK  $\hat{\Theta}(\theta) \triangleq \E_{(x,y) \sim \gD} \Theta(x, \theta)$. The condition number $\kappa \triangleq \lambda_\mathrm{max}/\lambda_\mathrm{min}$ serves as a metric to estimate the model ``trainability'' (\mie, how fast the model converges at early training stages)~\citep{ntk-metric}, with a smaller conditional number indicating higher trainability. 


\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/distribution.pdf}
    \caption{The conditional number of NTK versus the model performance (ACC) and vulnerability (ASR). \label{fig:scatter}}
\end{figure}


In our context, we consider the trigger generator and the target model as an end-to-end model and measure the empirical NTK of the trigger generator under randomly initialized $\theta$:
\begin{equation}
    \hat{\Theta}(\vartheta) \triangleq \E_{(x, y) \sim \gD, \theta \sim P_{\theta_\circ}}\,\left[\frac{\partial f( g(x; \vartheta);\theta)}{\partial \vartheta}\right] \left[\frac{\partial f(g(x; \vartheta;\theta)}{\partial \vartheta}\right]^\intercal %\quad J(x, \theta) \triangleq \frac{\partial f(x;\theta)}{\partial \theta}
\label{eq:score}
\end{equation}
where $P_{\theta_\circ}$ represents the initialization distribution of $\theta$. Here, we emphasize that the measure should be independent of $\theta$'s initialization.

Intuitively, $\hat{\Theta}(\vartheta)$ measures the trigger generator's trainability with respect to a randomly initialized target model. The generator's trainability indicates the easiness of effectively generating input-aware triggers, implying the model's vulnerability to input-aware backdoor attacks. To verify the hypothesis, on the CIFAR10 dataset with the generator configured as in Appendix\,\msec{sec:appb}, we measure $\hat{\Theta}(\vartheta)$ with respect to 900 randomly generated arches as well as the model accuracy (ACC) on clean inputs and the attack success rate (ASR) on trigger-embedded inputs, with the results shown in Figure~\ref{fig:scatter}. Observe that the conditional number of  $\hat{\Theta}(\vartheta)$ has a strong negative correlation with ASR, with a smaller value indicating higher attack vulnerability; meanwhile, it has a limited correlation with ACC, with most of the arches having ACC within the range from 80\% to 95\%.

% represents expensive computational cost. One workaround is to apply the back-optimization approach~\citep{back-opt}, which re-defines $\theta_\alpha$ as the output of an incomplete optimization: 
% \begin{equation}
%     \theta_\alpha = \mathsf{opt}_\theta (\gL_\mathsf{trn} (\theta, \alpha), \varsigma)
% \end{equation}
% where $\mathsf{opt}$ is a specific optimization procedure (\meg, gradient descent) with a fixed number of steps ($\varsigma$), which avoids solving the inner objective exactly.

% $\gD_\mathsf{trn}$ is the training data, $\theta_0$ is the initial parameters (sampled from the distribution $P_{\theta_0}$. 

Leveraging the insights above, we present a simple yet effective genetic algorithm that searches for exploitable arches without training, as sketched in Algorithm~\ref{alg:attack}. It starts from a candidate pool $\gA$ of $n$ arches randomly sampled from a pre-defined arch space; at each iteration, it samples a subset $\gA'$ of $m$ arches from $\gA$, randomly mutates the best candidate (\mie, with the lowest score), and replaces the oldest arch in $\gA$ with this newly mutated arch. In our implementation, the score function is defined as the condition number of \meq{eq:score}; the arch space is defined to be the \nats search space~\citep{nas-bench}, which consists of 5 atomic operators \{{\em none}, {\em skip connect}, {\em conv $1\times1$}, {\em conv $3\times3$}, and {\em avg pooling $3\times3$}\}; and the mutation function is defined to be randomly substituting one operator with another. 
% At each epoch, we sample $m$ candidates from the pool $\mathcal{A}$ and select the one with smallest score defined in Equation\mref{eq:score} as the best candidate. The mutation function randomly chooses an edge and modifies it to be a different operation.



% \section{Motivation}
% \label{sec:motivation}


% \subsection{trajectory}

% \begin{table*}[!ht]{\footnotesize
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%   \setlength{\tabcolsep}{3pt}
%     \begin{tabular}{c|c|c|c|c|c}
%     Row first & None & Skip Connect & Conv 1x1 & Conv 3x3 & Avg Pool 3x3 \\
%     \hline
%     None & \makecell{ASR: 30.01/45.70 \\ ACC: 90.34/90.88 \\Score: 7.00/12.54} & & & & \\
%     \hline
%     Skip Connect & & & & & \\
%     \hline
%     Conv 1x1 & & & & & \\
%     \hline
%     Conv 3x3 & & & & & \\
%     \hline
%     Avg Pool 3x3 & & & & & \\
%     \end{tabular}
%     \caption{Trajectory results}}
% \end{table*}



% \subsection{Algorithm}


\begin{algorithm}[!ht]
\setstretch{1.1}
{\small
  \KwIn{$n$ -- pool size; $m$ -- sample size; $\mathrm{score}$ -- score function; $\mathrm{sample}$ -- subset sampling function; $\mathrm{mutate}$ -- arch mutation function;}
  \KwOut{exploitable arch}
  %\tcp{\footnotesize candidate pool}
  $\gA, \gS, \gT= [], [], []$  \tcp*{candidate archs, scores, timestamps}
  \For{$i \gets 1$ \KwTo $n$}{
    $\gA[i] \leftarrow$ randomly generated arch, $\gS[i] \leftarrow \mathrm{score}(\gA[i])$, 
    $\gT[i] \leftarrow 0$\;
  }
  $best \leftarrow 0$\;
  \While{maximum iterations not reached yet}{
    $i \leftarrow \arg\min_{k \in \mathrm{sample}(\gA, m)} \gS[k]$  \tcp*{best candidate}
    $j \leftarrow \arg\max_{k \in \gA} \gT[k]$  \tcp*{oldest candidate}
    $\gA[j] \leftarrow \mathrm{mutate}(\gA[i])$ \tcp*{mutate candidate}
    $\gS[j] \leftarrow \mathrm{score}(\gA[j])$ \tcp*{update score}
    $\gT \leftarrow \gT + 1, \gT[j] \leftarrow 0$ \tcp*{update timestamps}
    \lIf{$\gS[j]< \gS[best]$}{$best \leftarrow j$}
  }
\Return $\gA[best]$\;
  \caption{\attack Attack \label{alg:attack}}}
\end{algorithm}


% \begin{align}
% \ssub{\alpha}{*}  = \arg\min_{\alpha} \mathbb{E}_{(x, y) \sim \mathcal{T}} [ s(\ssub{f}{\alpha,\theta}(\ssub{G}{\ssub{\theta}{G}}(x));\alpha) - \lambda \cdot s(\ssub{f}{\alpha,\theta}(x); \alpha)]
% \end{align}


% \begin{algorithm}[!ht]{\small
%   \KwIn{training sample distribution $\mathcal{T}$; model $\ssub{f}{\alpha,\theta}$; model parameters -- $\theta$; model arch parameters -- $\alpha$; generator $\ssub{G}{\ssub{\theta}{G}}$; generator parameters -- $\ssub{\theta}{G}$; hyper-parameter -- $\lambda$; learning rate -- $lr$; target class -- $t$; clean accuracy threshold -- $\mu$}
  
%   \KwOut{poisoned arch -- $\ssub{\alpha}{*}$}
  
%   $\ssup{\alpha}{(0)} \leftarrow \mathrm{RandomInit}(\alpha)$\;
  
%   $BestASR = 0.0$\;
  
%   \While{not converged yet}{
    
%     \tcp{\footnotesize optimize supernet}
%     \ForEach{$(x, y) \sim \mathcal{T}$}{
%       $\ssup{\theta}{(k)} \leftarrow \mathrm{RandomInit}(\ssub{\theta}{G})$\;
      
%       $\ssup{\ssub{\theta}{G}}{(k)} \leftarrow \mathrm{RandomInit}(\theta)$\;
      
%       \ssub{s}{poison} \leftarrow s(\ssub{f}{\ssup{\alpha}{(k)},\ssup{\theta}{(k)}}\circ\ssub{G}{\ssup{\ssub{\theta}{G}}{(k)}}(x))\;
      
%       \ssub{s}{clean} \leftarrow s(\ssub{f}{\ssup{\alpha}{(k)},\ssup{\theta}{(k)}}(x))\;
      
%       s \leftarrow \ssub{s}{poison} - \lambda \cdot \ssub{s}{clean}\;
      
%       $\ssup{\alpha}{(k+1)} \leftarrow \ssup{\alpha}{(k)} - lr \cdot \frac{\partial s}{\partial \ssup{\alpha}{(k)}}$\;
      
%       $k \leftarrow k + 1$\;
%     }

%     \tcp{\footnotesize evaluation}
%     $\ssup{\alpha}{eval} \leftarrow \mathrm{clip}(\ssup{\alpha}{(k)})$\;
    
%     $\ssup{\theta}{eval} \leftarrow \arg\min_\theta \mathbb{E}_{(x, y) \sim \mathcal{T}} [\ell (\ssub{f}{\ssup{\alpha}{eval},\theta}(x), y)]$\;
    
%     \If{$acc(\ssub{f}{\ssup{\alpha}{eval},\ssup{\theta}{eval}}) > \mu$}{
%       $\ssup{\ssub{\theta}{G}}{eval} \leftarrow \arg\min_{\ssub{\theta}{G}} \mathbb{E}_{(x, y) \sim \mathcal{T}} [\ell (\ssub{f}{\ssup{\alpha}{eval},\ssup{\theta}{eval}} \circ \ssub{G}{\ssub{\theta}{G}}(x), t)]$\;
%       \lIf{$asr(\ssub{G}{\ssup{\ssub{\theta}{G}}{eval}}, \ssub{f}{\ssup{\alpha}{eval},\ssup{\theta}{eval}}) > BestASR$}{
%         $\ssub{\alpha}{*} \leftarrow \ssup{\alpha}{eval}$
%       }
%     }
%   }
% \Return $\ssub{\alpha}{*}$\;
%   \caption{\attack Attack \label{alg:attack}}}
% \end{algorithm}


==> NAS backdoor/prestuff.tex <==
%
%
% Commonly used packages, definitions, and notations
%
% Ting Wang
% inbox.ting@gmail.com
%
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% commonly used packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\proof\relax
\let\endproof\relax
\let\amalg\relax

\newcommand\hmmax{0}
\newcommand\bmmax{0}


\usepackage{amsthm}
\theoremstyle{definition}
\newtheorem{definition}{Definition}


\usepackage{epsfig,amsmath,amsfonts,epsfig,multirow,makecell,caption,soul,csquotes,color,wrapfig,subcaption,mathtools,bm,spverbatim,booktabs,tcolorbox,diagbox,todonotes}
\usepackage[e]{esvect}


\newcommand{\ntodo}[1]{\todo[fancyline, inline, bordercolor=white, color=yellow!40]{#1}}
\newcommand{\stodo}[1]{{\color{red}{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Figure and Table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\captionsetup[table]{format=plain,labelformat=simple,labelsep=period}
\def\tablename{Table}
\def\figurename{Figure}

\usepackage{caption}
\captionsetup[figure]{font=small}
\captionsetup[table]{font=small}
\captionsetup[algorithm]{font=small}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% algorithm2e
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\makeatletter
\newif\if@restonecol
\makeatother
\let\algorithm\relax
\let\endalgorithm\relax
\usepackage[boxed, ruled, vlined, linesnumbered]{algorithm2e}
\SetKwRepeat{Do}{do}{while}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% space trick
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\setlength{\textfloatsep}{0.25\baselineskip}
\setlength{\floatsep}{0.3\floatsep}
\setlength{\dblfloatsep}{0.3\dblfloatsep}
\setlength{\dbltextfloatsep}{0.3\dbltextfloatsep}
\setlength{\intextsep}{0.3\intextsep}

\setlength{\belowcaptionskip}{4pt}
\setlength{\abovecaptionskip}{4pt}


\newenvironment{changemargin}[2]{\begin{list}{}{
	\setlength{\topsep}{0pt}\setlength{\leftmargin}{-8pt}
	\setlength{\rightmargin}{0pt}
	\setlength{\listparindent}{\parindent}
	\setlength{\itemindent}{\parindent}
	\setlength{\parsep}{0pt plus 1pt}
	\addtolength{\leftmargin}{#1}\addtolength{\rightmargin}{#2}
	}\item}
	{\end{list}}

\newenvironment{mitemize}{
	\begin{changemargin}{-5pt}{-0cm}
	\vspace{-15pt}
	\hspace{-15pt}
	\begin{itemize}
	\setlength{\itemsep}{3pt}}
	{\end{itemize}
	\vspace{2pt}
	\end{changemargin}}

\newenvironment{mdescription}{
	\begin{changemargin}{-8pt}{-0cm}
	\vspace{-13pt}
	\hspace{5pt}
	\begin{description}
	\setlength{\itemsep}{-1pt}}
	{\end{description}
	\end{changemargin}}

\newenvironment{menumerate}{
	\begin{changemargin}{-8pt}{-0cm}
	\vspace{-13pt}
	\hspace{5pt}
	\begin{enumerate}
	\setlength{\itemsep}{1pt}}
	{\end{enumerate}
	\end{changemargin}}

\newcommand{\mpara}[1]{\vspace{-6pt}\paragraph*{#1}}


\newcommand{\ssup}[2]{{#1}^{\scaleobj{0.8}{#2}}}
\newcommand{\ssub}[2]{{#1}_{\scaleobj{0.8}{#2}}}
\newcommand{\sboth}[3]{{#1}_{\scaleobj{0.8}{#2}}^{\scaleobj{0.8}{#3}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  space around titles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\usepackage{titlesec}
%\titlespacing\section{0pt}{6pt}{4pt}
%\titlespacing\subsection{0pt}{4pt}{3pt}
%\titlespacing\subsubsection{0pt}{3pt}{2pt}
%\titleformat{\subsection}{\large\bfseries}{\thesubsection}{1em}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%  gray colored cell for tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage[first=0,last=9]{lcg}
\usepackage{colortbl}
\definecolor{Gray}{gray}{0.8}
\colorlet{Red}{red!10!white}
\colorlet{Blue}{blue!10!white}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% definitions, lemmas, proofs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{prop}{Proposition}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% fancy section symbol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{hyperref}
\renewcommand{\sectionautorefname}{\S}
\newcommand{\msec}[1]{\S\,\ref{#1}}
\newcommand{\mref}[1]{\,\ref{#1}}
\newcommand{\meq}[1]{Eq.~\ref{#1}}
\newcommand{\mcite}[1]{\,\cite{#1}}
\newcommand{\met}{\;\textit{et al.}\xspace}
\newcommand{\mbackslash}{\scaleobj{0.6}{\backslash}}
\newcommand{\mct}[1]{({\it #1})}
\newcommand{\meg}{{\it e.g.}\xspace}
\newcommand{\mie}{{\it i.e.}\xspace}
\newcommand{\mcf}{{\it cf.}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% stirling

\DeclareRobustCommand{\stirling}{\genfrac\{\}{0pt}{}}
\newcommand{\com}[2]{C_{#1}^{#2}}

%%% smaller symbols

\usepackage{scalerel}[2016/12/29]

%%% leadto

\makeatletter
\providecommand{\leadsfrom}{%
  \mathrel{\mathpalette\reflect@squig\relax}%
}
\newcommand{\reflect@squig}[2]{%
  \reflectbox{$\m@th#1\leadsto$}%
}
\makeatother

%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rrm{{\textnormal{m}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.

\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> background.tex <==

\section{Preliminaries}
\label{sec:background}

We first introduce a set of key concepts and assumptions. 
%Table\mref{tab:notations} summarizes the important notations.

% \subsection{Neural Architecture Search}

% Deep neural networks (\dnns) represent a class of \ml models to learn high-level abstractions of complex data. We assume a predictive setting, in which a \dnn $\ssub{f}{\theta}$ (parameterized by $\theta$) encodes a function $\ssub{f}{\theta}: \ssup{\sR}{n} \rightarrow \ssup{\sS}{m}$, where $n$ and $m$ denote the input dimensionality and the number of classes. Given input $x$, $f(x)$ is a probability vector (simplex) over $m$ classes. 

% In this paper, we mainly focus on one primary task of \automl, 

% Neural architecture search (\nas) searches for performant \dnn architectures for given tasks~\citep{automl-survey}. Formally, let $\gD$ be the given dataset, $\ell(\cdot, \cdot)$ be the loss function, $\gF$ be the functional space of possible models (\mie, search space), the \nas method $\emA$ searches for a performant \dnn $\ssup{f}{*}$ via minimizing the following objective: 
% \begin{equation}
% \ssup{f}{*} = \arg\min_{f \in \gF} \E_{(x, y) \sim \gD} \, \ell(f(x), y)
% \end{equation}

% The existing \nas methods can be categorized according to their search spaces and strategies. In the following, we focus on the space of cell-based architectures~\citep{nasnet,enas,darts,snas,amoebanet}, which repeat the motif of a cell structure in a pre-specified arrangement, and the strategy of differentiable \nas\citep{darts,sgas,drnas}, which jointly optimizes the architecture and model parameters using gradient descent, due to their state-of-the-art performance and efficiency. % Nevertheless, our discussion generalizes to alternative \nas frameworks (details in \msec{sec:literature}). 
% We use {\darts}~\citep{darts} as a concrete example to illustrate differentiable \nas. 
% At a high level, \darts searches for two cell structures (\mie, normal cell and reduction cell) as the basic building blocks of the final architecture. A cell is modeled as a directed acyclic graph, in which each node $\ssup{x}{(i)}$ is a latent representation and each directed edge $(i,j)$ represents an operation $\ssup{o}{(i,j)}$ applied on $\ssup{x}{(i)}$ (\meg, skip connect). Each node is computed based on all its predecessors:
% \begin{equation}
%     \ssup{x}{(j)} = \sum_{i < j} \ssup{o}{(i,j)}(\ssup{x}{(i)})
% \end{equation}
% Each cell contains $\ssub{n}{\mathrm{in}}$ input nodes (often $\ssub{n}{\mathrm{in}}=2$), $\ssub{n}{\mathrm{out}}$ output nodes (often $\ssub{n}{\mathrm{out}} = 1$), and $\ssub{n}{\mathrm{mid}}$ intermediate nodes. Each input node takes the output from a preceding cell, the output node aggregates the latent representations from intermediate nodes, while each intermediate node is connected to $m$ preceding nodes (typically $m = \ssub{n}{\mathrm{in}}$). 
% %\ren{The illustration about intermediate nodes is confusing.}

% To enable gradient-based optimization of the architecture, \darts applies continuous relaxation on the search space. Letting $\gO$ be the set of candidate operations, the categorical choice of an operation is reduced to a softmax over $\gO$: 
% \begin{equation}
% \label{eq:softmax}
%     \ssup{\bar{o}}{(i,j)}(x) = \sum_{o \in \gO} \frac{\exp (\sboth{\alpha}{o}{(i,j)}) }{\sum_{o' \in \gO} \exp( \sboth{\alpha}{o'}{(i,j)})} o(x) 
% \end{equation}
% where $\sboth{\alpha}{o}{(i,j)}$ represents the trainable weight of operation $o$. When the search completes, a discrete architecture is obtained by replacing $\ssup{\bar{o}}{(i,j)}$ with the most likely operation $\arg\max_o \sboth{\alpha}{o}{(i,j)}$.

% The search is thus formulated as a bi-level optimization objective function: 
% \begin{equation}
% \label{eq:search}
% \min_\alpha\; \ssub{\gL}{\mathrm{val}} ( \ssup{\theta}{*}(\alpha), \alpha )    \quad \mathrm{s.t.} \quad \ssup{\theta}{*}(\alpha) = \arg\min_\theta \; \ssub{\gL}{\mathrm{trn}} (\theta, \alpha) 
% \end{equation}
% where $\ssub{\gL}{\mathrm{trn}}$ and $\ssub{\gL}{\mathrm{val}}$ are the training and validation losses, and $\alpha = \{\ssup{\alpha}{(i,j)}\}$ and  $\theta$ denote the architecture and model parameters, respectively. To handle the prohibitive cost of the nested optimization, single-step gradient descent is applied to avoid solving the inner objective exactly.
%while in {\drnas}\mcite{drnas}, the architecture parameters are modeled using a Dirichlet distribution to facilitate the optimization.

\subsection{Neural Tangent Kernel}




In \nas, it is necessary to evaluate the performance of candidate models. A na\"{i}ve way is to train the model from scratch to assess its performance, which can be extremely expensive. Recent work~\citep{nas-no-train,Wu:icea:2021,Abdelfattah:iclr:2021,Ning:nips:2021} has explored using easy-to-compute metrics as a proxy (without actual training). Most relevant to us, Chen {\em et al.} apply {\em neural tangent kernel} (NTK) to estimate the model ``trainability'' in terms of how fast the model training converges~\citep{ntk-metric}. 

Specifically, NTK describes the dynamics of DNN training by gradient descent~\citep{ntk,wide-dnn}. On the infinite width limit of DNNs, NTK becomes constant, which allows closed-form statements to be made about model training. Formally, considering given model $f$ (parameterized by $\theta$) as a map from input $x$ to a probability vector $f(x; \theta)$ over different classes, its Jacobian is defined as:
\begin{equation}
    J(x, \theta) \triangleq \frac{\partial f(x;\theta)}{\partial \theta}
\end{equation}
The NTK is then defined as the square matrix of: 
\begin{equation}
    \Theta(x, \theta) \triangleq J J^\intercal
\end{equation}
In practice, the condition number $\kappa = \frac{\lambda_{max}}{\lambda_{min}}$ of the empirical NTK matrix $\hat{\Theta}(\theta) \triangleq \E_{(x,y) \sim \gD} \Theta(x, \theta)$ is used as a metric to estimate the model trainability~\citep{ntk-metric}, with smaller conditional numbers indicating higher trainability. 
    

% by calculating its condition number. We design our attack based on this metric because it is differentiable w.r.t. model parameters.


% Neural Tangent Kernel (NTK) has been well studied to describe the dynamic evolution of DNNs during training stages).

% We have model $f$ that maps input $x$ and model parameters $\theta \in \mathbb{R}^{D}$ to a classification probability vector $f(x;\theta) \in \mathbb{R}^C$, where $C$ is number of classes.

% Jacobian
% $J(x, \theta) \triangleq \frac{\partial f(x;\theta)}{\partial \theta}$
% is a $(C\times D)$ matrix.

% Neural Tangent Kernel $\Theta(x, \theta) \triangleq J J^T$. It's a square matrix with shape $(C\times C)$.



% We evaluate the condition number $\kappa = \frac{\lambda_{max}}{\lambda_{min}}$ of empirical NTK matrix $\hat{\Theta}(\theta) \triangleq \mathbb{E}_{(x,y) \sim \mathcal{T}} [\Theta(x, \theta)]$



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

